Dynamics of Hot QCD Matter 2024 -- New facilities and instrumentation

This part of the conference proceeding provides a detailed overview of cutting-edge advancements in detector technologies, focusing on their optimization, characterization, and applications in particle physics experiments. Building on the insights and developments presented at the Hot QCD Matter 2022 conference, this section of the Hot QCD Matter 2024 proceedings highlights significant advancements in detector technologies. The development of Low Gain Avalanche Diodes (LGADs) into Ultra-Fast Silicon Detectors is explored, demonstrating their potential for superior timing resolution in future high-energy experiments. Simulation studies of Micropattern Gaseous Detectors (MPGDs), including MICROMEGAS and Gas Electron Multiplier (GEM) detectors, provide insights into their performance under high-radiation environments using tools like ANSYS and GARFIELD$^{++}$. A novel GEM foil geometry is proposed for improved gain and durability. Characterization of semiconductor detectors, such as Monolithic MALTA pixel detectors and CMS prototype silicon sensors, is also presented, highlighting their radiation tolerance, imaging capabilities, and structural integrity. These studies underscore the critical role of silicon sensors in ensuring detector reliability and performance. Additionally, the J-PARC muon g-2/EDM experiment is reviewed, showcasing its precision measurements to test Standard Model predictions and explore potential physics beyond. By addressing the interplay between detector development, simulation, and characterization, this proceeding showcases a collective effort toward advancing detector technologies and their pivotal role in pushing the boundaries of modern particle physics.

==> Sachin_Rana/ws-ijmpe.tex <==
\section{Study of MPGD based MICROMEGAS using ANSYS and GARFIELD\texorpdfstring{$^{++}$}{++}}

%\footnote{For the title,
%try not to use more than 3 lines. Typeset the title in 10 pt
%Times roman, uppercase and boldface.}}

\author{Sachin Rana, A Sarkar}


\bigskip



\begin{abstract}
Micro pattern gaseous detectors (MPGDs) represents a cutting edge technology in detection of particles which is important for applications in particle physics, security screening and  medical imaging. These detectors utilize electrodes having small scale patterns, typically in the order of tens to hundreds of micrometers, to increase the efficiency and precision of gas-based particle detection. MICRO MEsh GAseous Structure (MICROMEGAS) is a type of MPGD which offers a high spatial resolution and sensitivity. The detector consists of a two region separated by metal mesh structure called as micromesh. Control parameters of micromegas detector includes materials used,
geometry and type of gases. There are various flaws in the detector, like ion back flow, gain stability, discharge and less transparency that are needed to address. Geometry of micromegas has been constructed using simulation software
Ansys and Garfield$^{++}$ . The variation of average electric field is studied by making the different geometries and best results are obtained. Various simulations are also done to study the transparency of the detector. 
\end{abstract}
%\vspace{-0.25cm}
\keywords{MPGD, Garfield$^{++}$, Ansys, Transparency}
%\ccode{PACS numbers:}
%\tableofcontents
%\vspace{-0.4cm}
\subsection{Introduction}
%\vspace{-0.2cm}
By advancement in the particle accelerators, researchers are continually seeking for more efficient detectors. Gas ionization is the method used by gaseous detectors, which are especially made to measure ionizing radiation. MPGD\cite{sauli1999micropattern} is a class of advance particle detectors used in various fields in Physics. Micromegas detectors is a type of MPGD which is a high precision gaseous detector works in proportional region. Micromegas are known for their spatial resolution. In fact, among all the MPGDs, micromegas has the best spatial resolution. In this work, we are trying to replicate the geometry of micromegas with the help of various simulation software and enhancing the gain. Initial study of average electric field in the different regions is done using Ansys followed by gain analysis of the detector using Mechanical APDL\cite{thompson2017ansys} and Garfield$^{++}$. Variation of various geometrical factors like hole size, strip width and width of the avalanche region are performed using different tools and the results are presented.
\vspace{-0.5cm}
\subsection{Defining the geometry of Micromegas using Ansys}
%\vspace{-0.15cm}
To construct the geometry of micromegas, we have used the Ansys Maxwell\cite{jorgensen2020overview} software. It is a comprehensive electromagnetic field simulation software which utilize the finite element method to solve the complex electromagnetic problems with great accuracy. Step by step geometry constructed using Ansys Maxwell is shown in Figure \ref{fig:myplot9}, Figure \ref{fig:myplot10}, Figure \ref{fig:myplot11} and Figure \ref{fig:myplot12}.
%\vspace{-0.4cm}
\begin{figure}[h!t]
    \centering
    \begin{minipage}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=3.2cm]{Sachin_Rana/13.png} 
        \caption{Defining single unit cell}
        \label{fig:myplot9}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=3.2cm]{Sachin_Rana/11.png} 
        \caption{Remove undesired part}
        \label{fig:myplot10}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=3.2cm]{Sachin_Rana/12.png} 
        \caption{Micromesh structure}
        \label{fig:myplot11}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=1.6cm, height=3.2cm]{Sachin_Rana/15.png} 
        \caption{Geometry of Micromegas}
        \label{fig:myplot12}
    \end{minipage}
\end{figure}
%\vspace{-0.6cm}
%\vspace{-0.15cm}
Construction of geometry of micromegas starts by defining the single unit cell for mesh structure and then its repetition will make complete micromesh. Then it is placed at the desired location to separate drift and avalanche region. Complete geometry of micromegas is shown in Figure \ref{fig:myplot12}. Ansys Maxwell is used for the studies related to electric and magnetic field configurations. For the analysis related to gain, the geometry is constructed using Ansys Mechanical APDL. Geometry\cite{zhang2007simulation} constructed using APDL is shown in Figure \ref{fig:myplot13} and Figure \ref{fig:myplot14}.

 \begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=4.8cm, height=3.2cm]{Sachin_Rana/APDL1.png} 
        \vspace{-0.2cm}
        \caption{Geometry constructed using mechanical APDL via script writing. Thin green portion is micromesh.}
        \label{fig:myplot13}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=4.8cm, height=3.2cm]{Sachin_Rana/APDL2.png} 
        \vspace{-0.2cm}
        \caption{Complete meshing of the geometry which divides the simulation domain into smaller and discrete elements.}
        \label{fig:myplot14}
    \end{minipage}
\end{figure}

%\newline

In Figure \ref{fig:myplot13}, the small green region is the micromesh structure and the red regions below and above the micromesh are avalanche region and drift region respectively. The geometry is constructed using script writing. Figure \ref{fig:myplot14} is showing the meshing of complete geometry. It involves dividing the simulation domain into smaller, discrete elements that approximate the geometry and allow for solving physical equations over the model. After completing the construction part, Mechanical APDL generates four output files ELIST.lis, NLIST.lis, MPLIST.lis and PRSNOL.lis which contains information regarding material properties, nodes, meshing and potentials. In the next step we import these files to an another software named Garfield$^{++}$\cite{ciubotaru2018new} which is a C++ based simulation toolkit used for the optimization of gaseous ionization detectors. 
%Garfield$^{++}$
%\vspace{-0.4cm}
\subsection{Results and discussions}
%\vspace{-0.1cm}
The purpose of this work is to find the best configuration and to find the optimal parameters for the smooth working of micromegas. Firstly we observed the variation of average electric field for both drift  and avalanche region with hole size keeping strip width and the voltages at all three electrodes constant. We have found that the average electric field in drift region increase with increase in the hole diameter and average electric field is decreasing with increase in hole diameter in avalanche region. This is due to the fact that if we are increasing the hole size then there is a leakage of electric field from avalanche region to drift region.
%\vspace{-0.65cm}
\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=6.4cm, height=4.2cm]{Sachin_Rana/c3.pdf} 
        \caption{Average Electric Field in Drift Region as function of Hole Size at Strip width of 15\(\mu\)m }
        \label{fig:myplot}  % Unique label for this figure
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=6.4cm, height=4.2cm]{Sachin_Rana/c2.pdf} 
        \caption{Average Electric Field in Avalanche Region as function of Hole Size at Strip width of 15\(\mu\)m}
        \label{fig:myplot1}  % Unique label for this figure
    \end{minipage}
\end{figure}

The behavior is shown in Figure~\ref{fig:myplot} and Figure~\ref{fig:myplot1} respectively. To confirm this behavior, same study has been done for three different strip width. The behavior of electric field for varying hole size is shown in Figure~\ref{fig:myplot2} and Figure~\ref{fig:myplot3}.

\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=6.4cm, height=4.2cm]{Sachin_Rana/c.pdf} 
        \caption{Average Electric Field in Drift Region vs Hole Size for three different strip width. Red, green and blue lines denote the Strip width of 15\(\mu\)m, 20\(\mu\)m and 25\(\mu\)m respectively.}
        \label{fig:myplot2}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=6.4cm, height=4.2cm]{Sachin_Rana/c1.pdf} 
        \caption{Average Electric Field in Avalanche Region vs Hole Size for three different strip width. Blue, green and red lines denote the Strip width of 15\(\mu\)m, 20\(\mu\)m and 25\(\mu\)m}
        \label{fig:myplot3}
    \end{minipage}
\end{figure}

Figure~\ref{fig:myplot2} confirms that average electric field in drift region increases as we increase the hole size and Figure~\ref{fig:myplot3} gives the confirmation that average electric in avalanche region decrease as we increase the hole size. Apart from that, the behavior of average field is also studied for varying width of the avalanche region. The result obtained is shown in Figure~\ref{fig:myplot5}.
%\vspace{-0.6cm}
\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=6.4cm, height=4.2cm]{Sachin_Rana/c4.pdf} 
        \caption{Average Electric Field in Avalanche Region vs width of Avalanche region}
        \label{fig:myplot5}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=6.4cm, height=4.0cm]{Sachin_Rana/AV.png} 
        \caption{Ionization process inside the GEM geometry, studied using Garfield$^{++}$} 
        \label{fig:myplot6}
    \end{minipage}
\end{figure}
%\vspace{-0.4cm}
Smaller the width of the avalanche region small will be the gain. Here we can see that the average electric field is decreasing as we are increasing the width of the avalanche region.
%\vspace{-0.6cm}
\subsection{Gain calculation:}
%\vspace{-0.1cm}
The gain for micromegas depends on the detector's  geometry as well as the environmental factors. Theoretically, it is given as:
%\vspace{-0.3cm}
\newline
\begin{center}
%\vspace{-0.5cm}
    G = e$^{ad}$ with $\alpha$=APe$^{-BP/E}$
\end{center}
%\vspace{-0.35cm}
where d is the width of avalanche region and $\alpha$ is first Townsend coefficient. E is given as:
%\vspace{-0.4cm}
\begin{center}
    E=V$_{mesh}$/d
\end{center}

A and B are the coefficient depending on the gas mixture. P being the pressure of the gas. V$_{mesh}$ is the voltage at micromesh.\\
%Now for the gas mixture 90\% argon and 10\% CO$_2$ at 1bar pressure, the value of A and B are A=15cm$^{-1}$bar$^{-1}$ and B=230Vcm$^{-1}$bar$^{-1}$. Substituting all the values to calculate gain we get:
%\newline
%\begin{center}
 %   G=1.215
%\end{center}
%Now in real practice, the of micromegas has higher gain and it can be obtained by taking large potential difference and making suitable changes in the geometry.
\textbf{Gain calculation using Garfield$^{++}$}: With the help of Garfield$^{++}$, one can simulate the process of gas ionization. The avalanche process obtained using Garfield$^{++}$ is shown in Figure~\ref{fig:myplot6}. Here, in this figure the red and yellow lines are the ions and electrons produced in the avalanche process respectively. The two rectangular white strips are the part of micromesh. Red lines going above this part are the ion backflow. For the pitch size of 50$\mu$m and hole diameter of 30$\mu$m the gain value obtained using Garfield$^{++}$ is 450. 

\subsection{Summary and Conclusions:}

In this study, we examined how electric field behaves in different regions of the detector. Investigation on the variation of the hole size and strip width of the micromesh was conducted to observe their effects on the electric field. Simulations were performed using Ansys and Garfield$^{++}$ to evaluate the gain of the detector. These findings provides insights into optimizing the detector's geometry for improved performance.
%Geometry of micromegas has been constructed and behavior of electric field has been studied for the different geometrical configurations using Ansys and Garfield$^{++}$. Results obtained in this study are according to the expectations. Gain calculation has also done using Garfield$^{++}$.  

